WZ production cross-section measurement at 7 TeV and 8 TeV center of mass energies within the Compact Muon Solenoid experiment

The WZ associated diboson production is studied by measuring both inclusive cross section and, for the first time, the ratio between the $W^-Z$ and the $W^+Z$ cross sections. The measurements are performed using data samples of proton-proton collisions collected during the years 2011 and 2012, at 7 and 8 TeV of centre-of-mass energies, respectively, by the CMS experiment at the LHC, updating the 7 TeV cross section measurement available in CMS, and presenting the new cross section measurement in CMS at 8 TeV. The data sample used for the 7 TeV measurements correspond to an integrated luminosity of 4.9 $fb^{-1}$, whence the data for the 8 TeV correspond to $\mathcal{L}_{int}=19.6~fb^{-1}$. The obtained results are found compatible with the Standard Model predictions.

==> Makefile <==
VERSION=
LATEXTARGET=PhDThesis$(VERSION)

#
# LaTeX Makefile
# --------------
#
# Author : Jordi Duarte Campderros duarte@ifca.unican.es
#          based in original from s.m.vandenoord@student.utwente.nl (Stefan van den Oord)
# Date   : April 19, 2013.
# 
# This Makefile is a generic makefile for LaTeX documents. Distribute it
# as you wish, but please don't edit or remove this initial comment.
#
# The Makefile can be used by setting the environment variable "MAKEFILES",
# e.g. export MAKEFILES=~/data/TeX/Makefile.
# It requires GNU Make and bash or better, like zsh. Simply sh is not
# sufficient, I believe. The first few lines of the Makefile contains
# the executables that are used, edit them to point to the executables
# on your system.
#
# DISCLAIMER: Using this Makefile is fully at your own risk. I am not
#             responsible for anything! So if crucial files are removed
#             by the Makefile, it is your own problem. But you should
#             have backups anyway. :-)
#
# Usage
# -----
# The Makefile can do the following things for you:
# - generate PostScript equivalents of XFig figures;
# - run makeindex and BibTeX, but only if necessary;
# - compile the .dvi file, running LaTeX as many times as needed;
# - run XDvi with the compiled .dvi file;
# - create a PostScript equivalent of the .dvi file;
# - generate a HTML equivalent of the .dvi file (if Latex2HTML is
#   installed);
# - remove all generated output.
# The Makefile is in some points even RCS aware.
#
# In many cases, you don't even have to tell the Makefile which LaTeX
# file it has to compile. The Makefile uses the following strategy:
# 1. Check if the environment variable LATEXTARGET is set; if it is,
#    generate $LATEXTARGET.dvi.
# 2. If there is only one .tex file, use that one.
# 3. Check if there is a LaTeX file that has the same basename as the
#    directory. For example, if the directory is named "Thesis" and
#    there is a file "Thesis.tex", "Thesis.dvi" is generated.
#
# Invocation
# ----------
# When the MAKEFILES environment variable is set, you can use the
# following commands:
# - make latexhelp
#   Prints an overview of the available commands.
# - make latexfigures
#   Only generate the PostScript equivalents of XFig figures.
# - make file.dvi
#   Generates the specified DVI file.
# - make file.ps
#   Generates the DVI file and then runs dvips.
# - make latex
#   Use the above explained strategy to find out what has to be
#   generated, and generate it.
# - make view
#   Do a make latex and then run XDvi.
# - make latexps
#   Do a make latex and then run dvips.
# - make html
#   Do a make latex and then use LaTeX2HTML to create the HTML equivalent.
#   To do this, the following environment variables are used:
#   * HTMLDIR : the base dir in which the output is written. For example,
#               if HTMLDIR=~/public_html/LaTeX, and the file that is
#               generated is "Thesis", the output will be written in the
#               directory ~/public_html/LaTeX/Thesis.
#   * LATEX2HTML_OPTS : if you want to pass options to LaTeX2HTML, put
#                       them in this variable.
# - make latexclean
#   This command removes all generated output. CAUTION: the files that are
#   removed are thought out pretty well, but it is possible that files are
#   removed that you wanted to keep! Check below what files are removed if
#   you want to be certain!
#   Note that a file figure.eps is only removed if a file figure.fig exists.
#   (Even if the file figure.fig exists, but is checked in using RCS, the
#   file figure.eps will be removed.)
#
# Tip
# ---
# For some projects it is useful to have a separate Makefile in the project's
# directory. For example, when you use RCS, you could add functionality for
# automatic checkouts of the right files (adding dependencies is sufficient;
# GNU Make rocks :-).
# The command "latexclean" is declared so that you can add your own
# functionality in the project's Makefile; instead of one colon, declare it
# with two colons if you want to do that.
# For example:
# latexclean::
#     rm -f foo.bar
# This way both the origional definition in this Makefile and your own are
# used.

#.SILENT:

# SHELL=/usr/local/bin/bash

LATEX=latex
PDFLATEX=pdflatex
BIBTEX=bibtex
DVIPS=dvips
MAKEINDEX=makeindex
MAKEGLOSSARIES=makeglossaries
DVIVIEWER=xdvi -geometry 710x950-0+10
LATEX2HTML=latex2html

FIGURES=$(wildcard *.fig)
FIGUREOBJS=$(FIGURES:.fig=.eps)

TEXFILES=$(wildcard *.tex)

# Disable standard pattern rule:
%.dvi: %.tex

# Do not delete the following targets:
.PRECIOUS: %.aux %.bbl %.eps %.ind

%.aux: %.tex $(FIGUREOBJS) $(TEXFILES)
	@$(LATEX) $*
# Look for citations. Make sure grep never returns an error code.
	@grep "^\\\\citation" *.aux > .btmp.new || true

# If the citations are not changed, don't do anything. Otherwise replace
# the .btmp file to make sure Bibtex will be run.
	@if ( diff .btmp.new .btmp >& /dev/null ); then \
		rm .btmp.new; \
	else \
		mv .btmp.new .btmp; \
	fi

	@if [ -f $*.idx ]; then cp $*.idx .itmp.new; else touch .itmp.new; fi
	@if ( diff .itmp.new .itmp >& /dev/null ); then \
		rm .itmp.new; \
	else \
		mv .itmp.new .itmp; \
	fi

.btmp:

%.bbl: $(BIBFILES) .btmp
# Only use BibTeX if \bibliography occurs in the document. In that case,
# run BibTeX and recompile. .btmp is touched to prevent useless making
# next time.
	@if ( grep "^\\\\bibliography{" $*.tex > /dev/null ); then \
		$(BIBTEX) $*; \
		touch .rerun; \
	fi
	@touch .btmp

.itmp:

%.ind: .itmp
	@if [ -f $*.idx ]; then \
		#$(MAKEINDEX) $*; \
		touch .rerun; \
		touch .itmp; \
	fi

%.eps:%.fig
	@echo Generating figure $@...
	@fig2dev -L ps $< $@

%.dvi: %.aux %.ind %.bbl
# Make sure the dvi-file exists; if not: recompile.
	@if [ ! -f $*.dvi ]; then \
		touch .rerun; \
	fi

	@if [ -f .rerun ]; then \
		rm .rerun; \
		$(LATEX) $*; \
	else \
		$(MAKE) $*.aux; \
	fi

# While references et al. are changed: recompile.
	@while ( grep Rerun $*.log > /dev/null ); do \
		$(LATEX) $*; \
	done

# Touch the figureobjects to prevent making next time
	@if [ -n "$(FIGUREOBJS)" ]; then \
		touch $(FIGUREOBJS); \
		touch $*.aux; \
	fi

	@if [ -f $*.ind ]; then \
		touch $*.ind; \
	fi
	#@$(MAKEINDEX) -s nomencl.ist -o $*.nls $*.nlo
	#@$(MAKEGLOSSARIES) $<

latex:
# Below the 'true' is included to prevent unnecessarily many errors.
	@if [ -n "${LATEXTARGET}" ]; then \
		$(MAKE) ${LATEXTARGET}.dvi; \
		true; \
	else \
		if [ `ls *.tex | wc -l` = "1" ]; then \
			$(MAKE) `basename \`ls *.tex\` .tex`.dvi; \
			true; \
		else \
			$(MAKE) `echo $$PWD|tr '/' '\n'|tail -1`.dvi; \
			true; \
		fi; \
	fi

latexfigures:
	@for i in $(FIGUREOBJS); do \
		$(MAKE) $$i; \
	done

view:
# Below the 'true' is included to prevent unnecessarily many errors.
	@if [ -n "${LATEXTARGET}" ]; then \
		$(MAKE) ${LATEXTARGET}.dvi && \
		$(DVIVIEWER) ${LATEXTARGET}.dvi ; \
		true; \
	else \
		if [ `ls *.tex | wc -l` = "1" ]; then \
			$(MAKE) `basename \`ls *.tex\` .tex`.dvi && \
			$(DVIVIEWER) `basename \`ls *.tex\` .tex`.dvi; \
			true; \
		else \
			$(MAKE) `echo $$PWD|tr '/' '\n'|tail -1`.dvi && \
			$(DVIVIEWER) `echo $$PWD|tr '/' '\n'|tail -1`.dvi; \
			true; \
		fi; \
	fi

%.ps: %.dvi
	$(DVIPS) -o $*.ps $<
	#@$(MAKEINDEX) -s nomencl.ist -o $*.nls $*.nlo
	$(MAKEGLOSSARIES) $(patsubst %.tex, %, $<)
	$(DVIPS) -o $*.ps $<

# if any of the tex files has modified, just touch the main tex

%.pdf: *.tex Appendix/*.tex
	$(PDFLATEX) $(patsubst %.pdf,%, $@).tex
	#@$(MAKEINDEX) -s nomencl.ist -o $*.nls $*.nlo; 
	@$(MAKEGLOSSARIES) $(patsubst %.tex, %, $(patsubst %.pdf,%, $@)) 
	$(BIBTEX) $*
	$(PDFLATEX) $(patsubst %.pdf,%, $@)
	# Redoing glossaries to fix index 
	@$(MAKEGLOSSARIES) $(patsubst %.tex, %, $(patsubst %.pdf,%, $@)) 
	$(BIBTEX) $*
	$(PDFLATEX) $(patsubst %.pdf,%, $@)
	$(PDFLATEX) $(patsubst %.pdf,%, $@)
	

latexps:
	@if [ -n "${LATEXTARGET}" ]; then \
		$(MAKE) ${LATEXTARGET}.ps && \
		true; \
	else \
		if [ `ls *.tex | wc -l` = "1" ]; then \
			$(MAKE) `basename \`ls *.tex\` .tex`.ps && \
			true; \
		else \
			$(MAKE) `echo $$PWD|tr '/' '\n'|tail -1`.ps && \
			true; \
		fi; \
	fi

html: .html

.html:
	@if [ -n "${LATEXTARGET}" ]; then \
		if [ -n "${HTMLDIR}" ]; then \
			$(MAKE) ${LATEXTARGET}.dvi; \
			$(LATEX2HTML) $(LATEX2HTML_OPTS) -dir $(HTMLDIR)/$(LATEXTARGET) $(LATEXTARGET) && \
			chmod a+rx $(HTMLDIR)/$(LATEXTARGET) && \
			chmod a+r $(HTMLDIR)/$(LATEXTARGET)/* &&  \
			touch .html; \
		else \
			echo Set variable HTMLDIR\!; \
		fi; \
	else \
		echo Set variable LATEXTARGET\!; \
	fi

latexhelp:
	@echo "LaTeX Makefile Options"
	@echo "----------------------"
	@echo ""
	@echo "Environment variables:"
	@echo "  LATEXTARGET   Filename to make (without extension)"
	@echo "  HTMLDIR       Directory for HTML-output"
	@echo "  FIGURES       Figures that have to be compiled"
	@echo ""
	@echo "Targets:"
	@echo "  all           Make the LATEXTARGET or <dirname>.dvi"
	@echo "  <name>.dvi    Make the given dvi file"
	@echo "  latex         Make the LATEXTARGET or <dirname>.dvi"
	@echo "  view          Make and view the LATEXTARGET or <dirname>.dvi"
	@echo "  html          Make the LATEXTARGET  or <dirname>.dvi and generate HTML output"
	@echo "  latexhelp     This overview"
	@echo "  latexclean    Remove all generated files"

clean latexclean::
	@rm -f *.acl *.acn *.acr *.alg *.log *.aux *.dvi *.bbl *.blg *.ilg *.toc *.lof *.lot *.idx *.ind *.out *.brf *.html *.btmp *.itmp *.rerun *.glo *.glg *.gls *.nlo *.nls *.xdy *.slg *.slo *.sls
	@epsfiles=`find * -maxdepth 0  -name "*.eps" `; \
	if [ -n "$$epsfiles" ]; then \
		for i in *.eps; do \
			if [ -f `basename $$i .eps`.fig ]; then \
				rm -f $$i; \
			elif ( rcs `basename $$i .eps`.fig >& /dev/null ); then \
				rm -f $$i; \
			fi \
		done \
	fi
	@rm -f `find * -maxdepth 0  -name "*.[0-9]" ` `find * -maxdepth 0  -name "*.t[0-9]"` *.mp

cleanpspdf : clean
	@rm -f *.ps *.pdf

clobber : cleanpspdf
	@rm -f *~

